Safe Control for Nonlinear Systems Under Faults and Attacks Via Control Barrier Functions

Safety is one of the most important properties of control systems. Sensor faults and attacks and actuator failures may cause errors in the sensor measurements and system dynamics, which leads to erroneous control inputs and hence safety violations. In this paper, we improve the robustness against sensor faults and actuator failures by proposing a class of Fault-Tolerant Control Barrier Functions (FT-CBFs) for nonlinear systems. Our approach maintains a set of state estimators according to fault patterns and incorporates CBF-based linear constraints for each state estimator. We then propose a framework for joint safety and stability by integrating FT-CBFs with Control Lyapunov Functions. With a similar philosophy of utilizing redundancy, we proposed High order CBF-based approach to ensure safety when actuator failures occur. We propose a sum-of-squares (SOS) based approach to verify the feasibility of FT-CBFs for both sensor faults and actuator failures. We evaluate our approach via two case studies, namely, a wheeled mobile robot (WMR) system in the presence of a sensor attack and a Boeing 747 lateral control system under actuator failures.

==> sections/FeasibilityVerification_lastRev.tex <==
\subsection{Feasibility Verification}
\label{subsec:feasibility_verif}
In order for Theorem \ref{theorem:FT-HOCBF} to guarantee system safety, the linear constraint \eqref{eq:FT-CBF2} must hold for all time $t$. 
In what follows, we develop an SOS-based scheme to verify the feasibility of SCBF, FT-SCBF and FT-HOCBF constraints for both fault-free case and the case with sensor faults and attacks. 

% We present an SOS-based approach to verify the feasibility of an SCBF for both fault-free case and the case with sensor faults or attacks.  

% \textcolor{blue}{(1.5h) I think this paragraph needs to be rewritten. Perhaps say up front that you focus on verification for a constant-gain Kalman filter, and then state that this is the optimal Kalman filter (and hence satisfies the stochastic stability criteria) in the case where the system is LTI with constant noise.}

We focus on verification for a constant-gain Kalman filter. In the case where the system is LTI with constant noise, the steady-state Kalman filter gain is optimal and hence satisfies the stochastic stability criteria by Theorem \ref{theorem:EKF}. In this subsection, we omit the time subscript of $x_t$, $\hat{x}_t$ and $z_t$, i.e., ($x$, $\hat{x}$ and $z$) to simplify the expression. We consider an LTI system described by \eqref{eq:state-sde} and \eqref{eq:output-sde}, where $f(x)=F$, $g(x)=G$, the matrices $R_t = R$ and $Q_t=Q$.
For an LTI system, $P_t$ is the covariance matrix for the estimation error and will converge to a steady-state value $P$. The Kalman filter has a constant gain given by $K = Pc^{T}R^{-1}$. 
% For an nonlinear system, a constant gain extended Kalman filter is extensively studied by \cite{kobayashi2005application} and \cite{liu2017novel}. 
We introduce an SOS-based approach to verify the feasibility for this case. 

% For an nonlinear system, a constant gain extended Kalman filter is extensively studied by \cite{kobayashi2005application} and \cite{liu2017novel}. In this paper, we focus on the case with a constant Kalman filter gain instead of a time-varing gain. 
% We bypass the potential impact brought by time variant Kalman filter gain in this paper and present a special case with a constant gain. 
% \begin{Definition}[SCBF]
% \label{Def:SCBF}
%     For a system (\ref{eq:state-sde})--(\ref{eq:output-sde}) with safety region defined by (\ref{eq:safe-region}), the function $h$ is a \emph{Stochastic Control Barrier Function (SCBF)} of the system, if for all $x$ satisfying $h(x)>0$ there exists $u_t$ satisfying   
%     \begin{equation}
%     \label{eq:SCBF-1}
%     \frac{\partial h}{\partial x}(f(x_t)+g(x_t)u_{t}) - \frac{\partial h}{\partial x}(x_t)K_{t}c z_i 
%     + \frac{1}{2}\mathbf{tr}\left(\nu_{t}^{T}K_{t}^{T}\frac{\partial^{2}h}{\partial x^{2}}(x_t)K_{t}\nu_{t}\right) \geq -\alpha (h(x_t)).
%     \end{equation}
% \end{Definition}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Verifying feasibility of SCBF
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Verification for SCBF}
We first present the verification for an SCBF in an attack-free scenario, in which one SCBF-based safety constraint must be satisfied. We have the following initial result. 
\begin{proposition}
\label{prop:verify_scbf}
Suppose Assumption \ref{assumption:ekf} holds. The function $h(\hat{x})$ is a SCBF if and only if there is no $\hat{x}\in \mathcal{C}_{\gamma}$, $z\in\mathbb{R}^{n}$ satisfying
$\frac{\partial h}{\partial x}g(\hat{x}) = 0$ , $z^{T}z - \gamma^2 \leq 0$ and $\xi(\hat{x},z) < 0$ where 
\begin{multline}
\label{eq:prop2cond}
    \xi(\hat{x},z) =  \frac{\partial h}{\partial x}f(\hat{x}) +  \frac{1}{2}\mathbf{tr}\left(\nu^{T}K^{T}\frac{\partial^{2}h}{\partial x^{2}}(\hat{x})K\nu\right) + \\
\left\|\frac{\partial h}{\partial x}(\hat{x})K c \right\|_2 \gamma +  \hat{h}(\hat{x}).
\end{multline}
% \begin{multline}
% \label{eq:prop2cond}
%     \xi(\hat{x},z) =  \frac{\partial h}{\partial x}f(\hat{x}) +  \frac{1}{2}\mathbf{tr}\left(\nu^{T}K^{T}\frac{\partial^{2}h}{\partial x^{2}}(\hat{x})K\nu\right) + \\
% \frac{\partial h}{\partial x}(\hat{x})K c z +  \hat{h}(\hat{x}).
% \end{multline}
\end{proposition}
\begin{proof}
% By Theorem \ref{theorem:EKF}, we have $z^{T} z -\gamma^2 \leq 0$. By Definition \ref{Def:SCBF}, we have $\hat{h}(\hat{x}) = h(\hat{x})-\overline{h}_{\gamma}\geq 0$ for all $\hat{x}\in \mathcal{C}_{\gamma}:=\{x:\hat{h}(x)\geq 0\}$, \textcolor{blue}{if and only if $\dot{\hat{h}}(\hat{x})\geq0$ at the boundary}, i.e. when $\hat{h}(\hat{x})=0$. 
By Theorem \ref{theorem:SCBF}, the set $\mathcal{C}_{\gamma}$ is positive invariant given $\|x-\hat{x}\|\leq \gamma$ if for all time $t$ $u_t$ is chosen to satisfy \eqref{eq:SCBF-2} $\forall z_t$ with $\|z_t\|\leq \gamma$. By Definition \ref{Def:SCBF}, we have that $h(\hat{x})$ is a SCBF for all $\hat{x}\in \mathcal{C}_{\gamma}:=\{x:\hat{h}(x)\geq 0\}$, if and only if \eqref{eq:SCBF-2} holds at the boundary, i.e. when $\hat{h}(\hat{x})=0$. If $\frac{\partial h}{\partial x}g(\hat{x})\neq 0$, we can choose $u$ s.t. 
\begin{multline*}
\frac{\partial h}{\partial x}g(\hat{x}) u \geq \sup_{\|z\|\leq \gamma}\left\{-\frac{\partial h}{\partial x}f(\hat{x}) - \right. \\ \left. \frac{1}{2}\mathbf{tr}\left(\nu^{T}K^{T}\frac{\partial^{2}h}{\partial x^{2}}(\hat{x})K\nu\right) - 
\frac{\partial h}{\partial x}(\hat{x})K c z -  \hat{h}(\hat{x}) \right\} .
\end{multline*}
Since $\|z\|\leq \gamma$ is a compact set, such a $u$ always exists. Hence, (4) fails if and only if $\exists\hat{x}$ and $z$ with $\|z\|\leq \gamma$ s.t. (i) $\frac{\partial h}{\partial x}g(\hat{x})=0$, and (ii) $\xi(\hat{x},z)<0$ hold simultaneously. 
\end{proof}

Based on the proposition, we can formulate the following conditions via the Positivstellensatz. 
% \textcolor{red}{according change 20 mins}
\begin{Lemma}
A polynomial $h(\hat{x})$ is an SCBF for system (\ref{eq:state-sde})--(\ref{eq:output-sde}) 
if and only if there exist polynomials $\rho(\hat{x},z)$, sum-of-squares polynomials $q(\hat{x},z)$, integers $s$, $r_1$ and integer vectors $v$, $w$ such that
\begin{equation}
    \label{eq:verify_scbf}
    \phi(\hat{x},z) + \chi(\hat{x},z) + \psi(\hat{x}) = 0,
\end{equation}
and
\begin{align*}
    % f(\hat{x},z) &= \sum_{i=1}^{s} q_{i}(\hat{x},z)(-\xi(\hat{x},z)+z^{T}z-\gamma^2)b_i(\hat{x},z) \\
    \phi(\hat{x},z) &= \sum_{i=1}^{s} q_{i}(\hat{x},z)\left(-\xi(\hat{x},z)\right)^{v_i} \left(-z^{T}z+\gamma^2\right)^{w_i} \\
    \chi(\hat{x},z) &=  \left(\xi(\hat{x},z)\right)^{2 r_1}  \\
    \psi(\hat{x})  &= \sum_{i=1}^{m}\rho_i(\hat{x},z)\left[\frac{\partial h}{\partial x} g(\hat{x})\right]_{i},
\end{align*}
\end{Lemma}
\begin{proof}
By Proposition \ref{prop:verify_scbf}, we have $h(\hat{x})$ is an SCBF iff there exist no $\hat{x}$, $z$ such that$\frac{\partial h}{\partial x}g(\hat{x})=0$, $z^{T} z -\gamma^2 \leq 0$ and $-\xi(\hat{x},z)>0$. The latter two conditions are equivalent to $-z^{T} z +\gamma^2 \geq 0$, and $-\xi(\hat{x},z) \geq 0$, $\xi(\hat{x},z) \neq 0$. 
These conditions are equivalent to \eqref{eq:verify_scbf} by the Positivstellensatz.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Verifying feasibility of FT-SCBFs
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Verification for FT-SCBF}
We now extend the result into the case where sensors may experience faults and attacks. Specifically, we consider a nonlinear control system whose output may be affected by one of $m$ sensor faults described by \eqref{eq:sfstate-sde} and \eqref{eq:sfoutput-sde}. 

In this case, we need to verify the feasibility of $u$ to satisfy $m$ SCBF constraints under $m$ possible sensor faults.
To achieve this, we extend Proposition \ref{prop:verify_scbf} to verify the feasibility of a set of SCBF constraints via Farkas' Lemma. 

\begin{corollary}
\label{coro:Farkas}
Define $A(x)$ and $\Xi(x)$ as follows
\begin{equation}
    \begin{split}
    \label{coro1_AXi}
        A(x) &= \left( A_1(x) \ldots A_m(x) \right)^{T}, \\
        \Xi(x,z) &= [\xi_1(x,z) \ldots \xi_m(x,z)]^T.
    \end{split}
\end{equation}
Control input $u$ that chosen to satisfy a set of linear constraints, can be written as 
\begin{equation}
    \label{eq:coro1_u}
    A(x) u \leq \Xi(x,z). 
    % -\left[\frac{\partial h}{\partial x} g(x_j)\right]_i u_{j,i} \geq \xi(x_j)
\end{equation}
By Farkas's Lemma, the system $A(x) u \leq \Xi(x)$ has a solution $u\in\mathbb{R}^{p}$, if and only if there does not exist $y\in\mathbb{R}^{m}$ such that
\begin{equation}
    \label{eq:coro1_y}
    A^{T}(\hat{x})y=0, \ y\geq 0, \ \Xi^{T}(\hat{x},z)y<0.
\end{equation}
% $A^{T}(\hat{x})y=0$, $y\geq 0$ and $\Xi^{T}(\hat{x},z)y<0$.
\end{corollary}

We define $A(x)$ and $\Xi(x)$ as follows
\begin{equation*}
    \begin{split}
        A(\hat{x}) &= \left( -\frac{\partial h}{\partial x} g(\hat{x}_1) \ldots -\frac{\partial h}{\partial x} g(\hat{x}_{m}) \right)^{T}, \\
        \Xi(\hat{x},z) &= [\xi(\hat{x}_1,z) \ldots \xi(\hat{x}_{m},z)]^T.
    \end{split}
\end{equation*}

\begin{proposition}
\label{prop:verify_ftscbf}
Suppose Assumption \ref{assumption:ekf} and conditions in Theorem \ref{theorem:FT-HOCBF} hold.
There exists a feasible solution $u$ satisfying a set of $m$ SCBF constraints if and only if there is no $\hat{x}_1, \ldots, \hat{x}_{m}\in \mathcal{C}_{\gamma}$, $z_1, \ldots, z_{m}\in \mathbb{R}^n$ and $y\in \mathbb{R}^{m}$ satisfying $\frac{\partial h}{\partial x}g(\hat{x}_j)= 0$, $\forall j$, $(\hat{x}_i-\hat{x}_j)^T (\hat{x}_i-\hat{x}_j)- \gamma^2 \leq 0$, $\forall i,j$, $z_j^{T} z_j -\gamma^2 \leq 0 \ \forall j$, $A^{T}(\hat{x})y=0$, $y\geq 0$ and $\Xi^{T}(\hat{x},z)y<0$.
\end{proposition}
\begin{proof}
By Definition \ref{Def:SCBF}, we have $\hat{h}(\hat{x}_j) = h(\hat{x}_j)-\overline{h}_{\gamma}\geq 0$ for all $\hat{x}_j\in \mathcal{C}_{\gamma}$. By Theorem \ref{theorem:EKF}, we have $z_j^{T} z_j -\gamma^2 \leq 0$ for all $j$. 
By Theorem \ref{theorem:FT-HOCBF}, we have $(\hat{x}_i-\hat{x}_j)^T (\hat{x}_i-\hat{x}_j)\leq \gamma^2$, $\forall i,j$. 
For the case where $\hat{h}(\hat{x})=0$, $u$ can be chosen to satisfy \eqref{eq:SCBF-2} for all $j$. By Corollary \ref{coro:Farkas}, we have the existence of $u$ if and only if there does not exist $y\in\mathbb{R}^{m}$ such that \eqref{eq:coro1_y} hold.
Conversely, if for some $\hat{x}_0$, $\hat{x}_1$, $z_0$ and $y_0$ satisfying $\frac{\partial h}{\partial x}g(\hat{x}) = 0$, 
$(\hat{x}_0-\hat{x}_1)^T (\hat{x}_0-\hat{x}_1) - \gamma^2 \leq 0$, $z_0^{T} z_0 -\gamma^2 \leq 0 $, $A^{T}(\hat{x})y_0=0$, $y_0\geq 0$ and $\Xi^{T}(\hat{x},z)y_0<0$, the set $\mathcal{C}$ is not positive invariant.
% For the case where $\hat{h}(\hat{x})=0$, $u$ can be chosen to satisfy \eqref{eq:SCBF-2} for all $j$, which can be written as 
% \begin{equation}
%     \label{eq:ftscbf1_u}
%     A(\hat{x}) u \leq \Xi(\hat{x},z). 
%     % -\left[\frac{\partial h}{\partial x} g(x_j)\right]_i u_{j,i} \geq \xi(x_j)
% \end{equation}

% By Farkas's Lemma, the system $A u \leq \Xi$ has a solution $u\in\mathbb{R}^{p}$, if and only if there does not exist $y\in\mathbb{R}^{m}$ such that $A^{T}(\hat{x})y=0$, $y\geq 0$ and $\Xi^{T}(\hat{x},z)y<0$. 
% Conversely, if for some $\hat{x}_0$, $\hat{x}_1$, $z_0$ and $y_0$ satisfying $\frac{\partial h}{\partial x}g(\hat{x}) = 0$, $(\hat{x}_0-\hat{x}_1)^T (\hat{x}_0-\hat{x}_1)> \gamma^2$, $z_0^{T} z_0 -\gamma^2 > 0 $, $A^{T}(\hat{x})y_0=0$, $y_0\geq 0$ and $\Xi^{T}(\hat{x},z)y_0<0$, the set $\mathcal{C}$ is not positive invariant.
\end{proof}

Then we can formulate the following conditions via the Positivstellensatz.

\begin{Lemma}
\label{Lemma:verify_ftscbf}
There exists a feasible solution $u$ satisfying a set of $m$ SCBF constraints if and only if there exist polynomials $\rho(\hat{x}_j,y,z_j)$, sum-of-squares polynomials $q(\hat{x}_j,y,z_j)$, integers $s$, $r_1$, and integer vectors $v_i$, $w_i$, $l_i$, $m_i$, for all $i \in \{1,\ldots, s\}$ such that
\begin{equation}
    \label{eq:verify_ftscbf}
    \phi(\hat{x}_j,y,z_j) + \chi(\hat{x}_j, y,z_j) + \psi(\hat{x}_j,y,z_j) = 0, 
\end{equation}
and
\begin{align*}
    \phi(\hat{x}_j,y,z_j) =& \sum_{j=1}^{s}\sum_{i=1}^{s}  q_{i}(\hat{x}_j,y,z_j) 
    \left(-z_j^{T}z_j+\gamma^2\right)^{v_i}  \\
    & \left(-(\hat{x}_i-\hat{x}_j)^T (\hat{x}_i-\hat{x}_j)+ \gamma^2\right)^{w_i}\\
    & \left(\Xi^{T}(\hat{x},z)y\right)^{l_i} y^{m_i}  \\
    % \\ &\left[(-(\hat{x}_i-\hat{x}_j)^T (\hat{x}_i-\hat{x}_j)+ \gamma^2)+(z^{T}z-\gamma^2)-\Xi^{T}y+y \right] 
    % b_i(\hat{x}_j,y,z_j) \\
    \chi(\hat{x}_j, y,z_j) =& \left(\Xi^{T}(\hat{x},z)y\right)^{2 r_1}\\
    \psi(\hat{x}_j,y,z_j)  =& \sum_{j}^{l}\left( \sum_{i=1}^{m}\rho^0_i(\hat{x}_j,y,z_j)\left[\frac{\partial h}{\partial x} g(\hat{x})\right]_{i} + \right.\\
    & \left. \sum_{i=1}^{m}\rho^1_i(\hat{x}_j,y,z_j)\left[A^T(\hat{x}) y\right]_{i} \right),
\end{align*}
\end{Lemma}
\begin{proof}
By Proposition \ref{prop:verify_ftscbf}, we have $h(\hat{x})$ is an SCBF if and only if there exist no $\hat{x}_1, \ldots, \hat{x}_{m}$, $z_1, \ldots, z_{m}$ and $y$ satisfying $\frac{\partial h}{\partial x}g(\hat{x}) = 0$, $(\hat{x}_i-\hat{x}_j)^T (\hat{x}_i-\hat{x}_j)- \gamma^2 \leq 0$, $\forall i,j$, $z_j^{T} z_j -\gamma^2 \leq 0 \ \forall j$, $A^{T}(\hat{x})y=0$, $y\geq 0$ and $\Xi^{T}(\hat{x},z)y<0$. 
The conditions are equivalent to 
\begin{equation*}
    \begin{split}
    &\frac{\partial h}{\partial x}g(\hat{x}) = 0,\\
    &-(\hat{x}_i-\hat{x}_j)^T (\hat{x}_i-\hat{x}_j)+ \gamma^2 \geq 0, \forall i,j,\\ 
    & -z_j^{T} z_j +\gamma^2 \geq 0 , \forall j \\
    &A^{T}(\hat{x})y=0, \ y\geq 0, \ -\Xi^{T}(\hat{x},z)y\geq 0, \Xi^{T}(\hat{x},z)y\neq 0
    \end{split}
\end{equation*}
These conditions are equivalent to \eqref{eq:verify_ftscbf} by the Positivstellensatz.
\end{proof}

\subsubsection{Verification for FT-SCBF with high relative degree}
We further extend the proposition \ref{prop:verify_ftscbf} and Lemma \ref{Lemma:verify_ftscbf} to verify the feasibility of a set of HOSCBF constraints. 

We define $A(x)$ and $\Xi(x)$ as follows
\begin{equation*}
    \begin{split}
        A(\hat{x}) =& \left( -\frac{\partial h^{d^{\prime}}}{\partial x} g(\hat{x}_1), \ldots, -\frac{\partial h^{d^{\prime}}}{\partial x} g(\hat{x}_{m}) \right)^{T}, \\
        \Xi(\hat{x},z) =& [\xi(\hat{x}_1), \ldots, \xi(\hat{x}_{m})]^T, where \\
        \xi(\hat{x},z) =&  \frac{\partial h^{d^{\prime}}}{\partial x}f(\hat{x}) +  \frac{1}{2}\mathbf{tr}\left(\nu^{T}K^{T}\frac{\partial^{2}h^{d^{\prime}}}{\partial x^{2}}(\hat{x})K\nu\right) + \\
        & \ \frac{\partial h^{d^{\prime}}}{\partial x}(\hat{x})K c z +  \hat{h}^{d^{\prime}}(\hat{x}).
    \end{split}
\end{equation*}
% where 
% \begin{multline*}
%     \xi(\hat{x},z) =  \frac{\partial h^{d^{\prime}}}{\partial x}f(\hat{x}) +  \frac{1}{2}\mathbf{tr}\left(\nu^{T}K^{T}\frac{\partial^{2}h^{d^{\prime}}}{\partial x^{2}}(\hat{x})K\nu\right) + \\
%     \frac{\partial h^{d^{\prime}}}{\partial x}(\hat{x})K c z +  \hat{h}^{d^{\prime}}(\hat{x}).
% \end{multline*}

\begin{proposition}
\label{prop:verify_fthocbf}
Suppose Assumption \ref{assumption:ekf} and conditions in Theorem \ref{theorem:FT-HOCBF} hold.
There exists a feasible solution $u$ satisfying a set of $m$ HOSCBF constraints with relative degree $d$ if and only if there is no $\hat{x}_1, \ldots, \hat{x}_{m}\in \mathcal{C}_{\gamma}$, $z_1, \ldots, z_{m}\in \mathbb{R}^{n}$ and $y\in \mathbb{R}^{m}$ satisfying $\hat{h}^{d}(\hat{x_j})\geq 0, \ \forall j, \forall d\leq d^{\prime} $, $\frac{\partial h^{d^{\prime}}}{\partial x}g(\hat{x}_j)= 0$, $(\hat{x}_i-\hat{x}_j)^T (\hat{x}_i-\hat{x}_j)-  \gamma^2 \leq 0$, $\forall i,j$, $z_j^{T} z_j -\gamma^2 \leq 0 \ \forall j$, $A^{T}(\hat{x})y=0$, $y\geq 0$ and $\Xi^{T}(\hat{x},z)y<0$. 
\end{proposition}
\begin{proof}
By Theorem \ref{theorem:EKF}, we have $z_j^{T} z_j -\gamma^2 \leq 0$ for all $j$ with $m$ EKFs. 
By the Definition \ref{Def:HOSCBF}, we have $\hat{h}^{d}(\hat{x}_j) = h^{d}(\hat{x}_j)-\overline{h}_{\gamma}\geq 0$ for all $\hat{x}_j\in \overline{\mathcal{C}}$, if and only if the following three conditions are satisfied. For all $\hat{x}_j\in \overline{\mathcal{C}}$, $\hat{h}^{d}(\hat{x})\geq0$ for all $d\leq d^{\prime}$. Next, by Theorem \ref{theorem:FT-HOCBF}, $(\hat{x}_i-\hat{x}_j)^T (\hat{x}_i-\hat{x}_j)\leq \gamma^2$, $\forall i,j$. Moreover, $\frac{\partial h^{d^{\prime}}}{\partial x}g(\hat{x}_j)\neq 0$ and $u$ are chosen to satisfy \eqref{eq:hoscbf} for all $j$. By Corollary \ref{coro:Farkas}, we have a solution $u\in\mathbb{R}^{p}$ exists, if and only if there does not exist $y\in\mathbb{R}^{m}$ such that \eqref{eq:coro1_y} holds. 
Conversely, if for some $\hat{x}_0$, $\hat{x}_1$, $z_0$ and $y_0$ satisfying $\hat{h}^{d}(\hat{x}_0) \geq 0$, $(\hat{x}_0-\hat{x}_1)^T (\hat{x}_0-\hat{x}_1)- \gamma^2 \leq 0$, $z_0^{T} z_0 -\gamma^2 \leq 0 $, $A^{T}(\hat{x})y_0=0$, $y_0\geq 0$ and $\Xi^{T}(\hat{x},z)y_0<0$, the set $\mathcal{C}$ is not positive invariant. 
\end{proof}

\begin{Lemma}
\label{Lemma:verify_fthocbf}
There exists a feasible solution $u$ satisfying a set of $m$ HOSCBF constraints 
if and only if there exist polynomials $\rho(\hat{x}_j,y,z_j)$, sum-of-squares polynomials $q(\hat{x}_j,y,z_j)$, integers $s$, $r_1$, and integer vectors $n_1, \ldots, n_{d^{\prime}}$, $v_i$, $w_i$, $l_i$, $m_i$ for all $i \in \{1,\ldots, s\}$ such that
\begin{equation}
    \label{eq:verify_fthocbf}
    \phi(\hat{x}_j,y,z_j) + \chi(\hat{x}_j, y,z_j) + \psi(\hat{x}_j,y,z_j) = 0, 
\end{equation}
and
\begin{align*}
    \phi(\hat{x}_j,y,z_j) =& \sum_{j=1}^{s}\sum_{i=1}^{s} \left( q_{i}(\hat{x}_j,y,z_j)
    \left(-z_j^{T}z_j+\gamma^2\right)^{v_i} \right. \\
    & \left. \left(-(\hat{x}_i-\hat{x}_j)^T (\hat{x}_i-\hat{x}_j)+ \gamma^2\right)^{w_i} \right. \\
    & \left. \left(-\Xi^{T}(\hat{x},z)y\right)^{l_i} y^{m_i} \prod_{d=1}^{d^{\prime}}\left(\hat{h}^{d}(\hat{x})\right)^{n_d}\right) \\
    % \\ &\left[(-(\hat{x}_i-\hat{x}_j)^T (\hat{x}_i-\hat{x}_j)+ \gamma^2)+(z^{T}z-\gamma^2)-\Xi^{T}y+y \right] 
    % b_i(\hat{x}_j,y,z_j) \\
    \chi(\hat{x}_j, y,z_j) =& 
    \left(\Xi^{T}(\hat{x},z)y\right)^{2 r_1}\\
    \psi(\hat{x}_j,y,z_j)  =& \sum_{j}^{l}\left( \sum_{i=1}^{m}\rho^0_i(\hat{x}_j,y,z_j)\left[\frac{\partial h^{d^{\prime}}}{\partial x}g(\hat{x}_j)\right]_{i} + \right. \\
    & \left. \sum_{i=1}^{m}\rho^1_i(\hat{x}_j,y,z_j)\left[A^T(\hat{x}) y\right]_{i} \right),
\end{align*}
\end{Lemma}
\begin{proof}
By proposition \ref{prop:verify_fthocbf}, we have $h^{d}(\hat{x})$ are HOSCBFs if and only if there exist no $\hat{x}_1, \ldots, \hat{x}_{m}\in \mathcal{C}_{\gamma}$, $z_1, \ldots, z_{m}\in \mathbb{R}^{n}$ and $y\in \mathbb{R}^{m}$ satisfying $\hat{h}^{d}(\hat{x_j})\geq0, \ \forall j, \forall d\leq d^{\prime}$, $\frac{\partial h^{d^{\prime}}}{\partial x}g(\hat{x}_j)= 0$, $(\hat{x}_i-\hat{x}_j)^T (\hat{x}_i-\hat{x}_j)- \gamma^2 \leq 0$, $\forall i,j$, $z_j^{T} z_j -\gamma^2 \leq 0 \ \forall j$, $A^{T}(\hat{x})y=0$, $y\geq 0$ and $\Xi^{T}(\hat{x},z)y<0$. 
The conditions are equivalent to 
\begin{equation*}
    \begin{split}
    &\frac{\partial h^{d^{\prime}}}{\partial x}g(\hat{x}_j)= 0, \ \hat{h}^{d}(\hat{x_j})\geq0, \ \forall j, \forall d\leq d^{\prime}\\
    &-(\hat{x}_i-\hat{x}_j)^T (\hat{x}_i-\hat{x}_j)+ \gamma^2 \geq 0, \ \forall i,j,\\ 
    & -z_j^{T} z_j +\gamma^2 \geq 0, \ \forall j \\
    &A^{T}(\hat{x})y=0, \ y\geq 0, \ -\Xi^{T}(\hat{x},z)y\geq 0, \Xi^{T}(\hat{x},z)y\neq 0
    \end{split}
\end{equation*}
These conditions are equivalent to \eqref{eq:verify_fthocbf} by the Positivstellensatz.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
\subsection{FT-HOCBF Construction}
\label{subsec:CBF-construction}
We consider LTI systems with dynamics
\begin{equation}
\label{eq:LTI-SDE}
dx_{t} = (Fx_{t} + Gu_{t}) \ dt + \sigma dW_{t}. 
\end{equation}
We develop sufficient conditions for two cases of safe regions, defined by half-planes and ellipsoids, satisfying constraint \eqref{eq:FT-CBF2}.

\subsubsection{Half-plane Constraint with LTI System}
We first consider half-plane constraints with the form of $h(x)=a^T x -b$. The following lemma \cite{clark2021control} describes the structure of the $h^{i}(x)$.
\begin{Lemma}
\label{Lemma:halfplaneHOBF}
The function $h^{i}$ can be written in the form
\begin{multline*}
    h^{i}(x)=\sum_{d_{0}, \ldots, d_{i-1}} \beta_{i}^{d_{0}, \ldots, d_{i-1}, 0}\left(a^{T} F^{0} x\right)^{d_{0}}\left(a^{T} F^{1} x\right)^{d_{1}}\\ \cdots\left(a^{T} F^{i-1} x\right)^{d_{i-1}}+a^{T}F^{i}x
\end{multline*}
for some values of the coefficients $\beta^{d_0,\dots,d_i}$
\end{Lemma}
\begin{proof}
Since the system is controllable LTI system, there exists a minimum $i$ such that $a^{T}F^{i}G \neq 0$. Furthermore, $\frac{\partial h^{i}}{\partial x}Gu = a^{T}F^{i}Gu$.
We can choose an index $l \in \{1,\ldots,p\}$ such that $[a^{T}F^{i}G]_{l} \neq 0$, set $[u]_{s} = 0$ for $s \neq l$, and select $[u]_{l} > 0$ if $[a^{T}F^{i}G]_{l} > 0$ and $[u]_{l} < 0$ if $[a^{T}F^{i}G]_{l} < 0$. Hence a high relative degree half-plane constraint can be satisfied with the desired probability.
\end{proof}


% We choose class $\kappa$ function $\alpha_i$ as linear function with gain $k_i>0$ and $i$ indicating the corresponding relative degree and define the HOCBF with as follows
% \begin{equation*}
%     \begin{split}
%         h^0(x_t) &= a^T x_t -b\\
%         h^1(x_t) &= \Dot{h}^0(x_t) + k_1 h^0(x_t) \\
%         h^2(x_t) &= \Dot{h}^1(x_t) + k_2 h^1(x_t) \\
%         &\ldots \\
%         h^r(x_t) &= \Dot{h}^{(r-1)}(x_t) + k_r h^{(r-1)}(x_t).\\
%     \end{split}
% \end{equation*}
% Then, we can have $\nabla \hat{h}^{r}_j = k_{r}k_{r-1}\dots k_1 a^T$ and 
% $$\Lambda_{j}^r = \nabla \hat{h}^{r}_j G = k_{r}k_{r-1}\dots k_1 a^T G.$$
% Since we have all $k_i>0$, for $i=1,\dots, r$, we can consider the case where $a^{T}G \neq 0$ and $a^{T}G = 0$.
% \begin{Lemma}\cite{clark2020control}
% \label{lemma:half-plane-CBF}
% Suppose that $a^{T}G \neq 0$. Then at each time $t$, there exists $u$ satisfying (\ref{eq:FT-CBF2}).
% \end{Lemma}
% Next, we consider the case where $a^{T}G = 0$. If the LTI system is controllable, then there exists a minimum $i$ such that $a^{T}F^{i}G \neq 0$. 



\subsubsection{Ellipsoid Constraint with LTI System}
We next consider an ellipsoid constraint of the form $\mathcal{C} = \{x : (x-x^{\prime})^{T}\Phi(x-x^{\prime}) \leq 1\}$ for some positive definite matrix diagonalizable $\Phi$ and $x^{\prime} = 0$, so that $h(x) = 1 - (x-x^{\prime})^{T}\Phi(x-x^{\prime})$. 
We define
$$\hat{h}^{0}_{i}(\hat{x}) = 1-\overline{h}^{0}_{\gamma_{i}} - (x-x^{\prime})^{T}\Phi(x-x^{\prime}).$$
We assume matrix $F$ to be diagonalizable simultaneously for matrix multiplication commutative property to render cleaner expression. 
\begin{Lemma}
\label{Lemma:ellipsoidHOCBF}
For a controllable system defined by \eqref{eq:LTI-SDE} with positive-definite diagonalizable matrix $F$, we can have the derivative of function $\hat{h}^{d}_{j}(\hat{x})$ expressed as 
\begin{equation}
    \frac{\partial\hat{h}^{d}_{j}}{\partial x} = -2 \sum_{d=0}^{d'} \alpha^{0,1,\dots,d}_j 2^{d'-d}x^T \Phi F^{d'-d} 
\end{equation}
for some value of the coefficients $\alpha^{0,1,\dots,d}_j$.
\end{Lemma}
We omit the proof of Lemma \ref{Lemma:ellipsoidHOCBF} due to space. 
% We assume matrix $F$ and $\Phi$ to be diagonalizable simultaneously for matrix multiplication commutative property to render cleaner expression $\frac{\partial\hat{h}^{d}_{j}}{\partial x}$.
% \begin{Lemma}
% A high relative degree ellipsoid constraint can be satisfied with desired probability if $u$ satisfies $F^{r-l}Gu=-x$, where $l=min\{i\mid F^i G\neq 0\}$
% \end{Lemma}
% \begin{pf}
%     We further define $\Lambda^r_i=\frac{\partial\hat{h}^{d}_{j}}{\partial x}G$. There exist $l\in\{1,\dots,r\}$ such that $F^{r-l}G\neq0$ due to the controllability. 
%     We can select $u$ such that $F^{r-l}Gu=-x$.  
%     Then we can have $\Lambda^r_i G u$ in the form of sum of squares. 
%     $$\Lambda^r_i G u = 2 \sum_{i=0}^{d} \alpha_{0,1,\dots,i} 2^{r-i}x^T \Phi F^{r-i}x\geq0.$$
% \end{pf}
We further define $\Lambda^d_j=\frac{\partial\hat{h}^{d}_{j}}{\partial x}G$. There exists $l\in\{1,\dots,d'\}$ such that $F^{d'-l}G\neq0$ due to the controllability. 
We can select $u$ such that $F^{d'-l}Gu=-x$.  
Then we can have $\Lambda^d_j  u$ in the form of sum of squares. 
$$\Lambda^d_j  u = 2 \sum_{i=0}^{d'} \alpha^{0,1,\dots,i}_j 2^{d'-l}x^T \Phi x\geq0.$$
Hence, high relative degree ellipsoid constraint can be satisfied with desired probability
\fi
